Differentiability, Convenient Spaces and Smooth Diffeologies

We review the basic definitions and properties concerning smooth structures, convenient spaces, diffeological spaces and tangent structures. The relation betwen them is described. A tangent structure is constructed for each pre-convenient space. This one is proved to be convenient iff the space and the tangent fibres coincide. Some basic comments on the relation with manifolds are given.

==> RELB.TEX <==
\pageno=12


\font\eightrm=cmr8         %% for the abstract
\font\eightit=cmti8        %% for the abstract
\font\eightmi=cmmi8        %% math italics in abstract
\font\tensmc=cmcsc10       %% for the authors
\def\smc{\tensmc}          %% use small capitals

\def\opname#1{\mathop{\rm#1}\nolimits} %% = AmSTeX \operatorname

\def\frac#1#2{{#1\over #2}}   %% displayed fraction

\def\implies{\Rightarrow}
\def\N{{\bf N}}               %% nonnegative integers
\def\norm#1{\Vert#1\Vert}
\def\ox{\otimes}              %% tensor product
\def\pd#1#2{{\del #1\over\del #2}} %% partial derivative
\def\qed{\allowbreak\qquad\null
         \nobreak\hfill\square}%% end-proof marker at right
\def\R{{\bf R}}               %% real numbers
\def\set#1{\{\,#1\,\}}        %% set notation
\def\square{\vrule height 5pt depth 0pt
             width 5pt}       %% black square for \qed
\def\Supp{\opname{Supp}}

\def\W{\bigwedge}             %% exterior product space
\def\w{\wedge}                %% exterior product
\def\x{\times}                %% cartesian product
\def\.{\cdot}                 %% group action
\def\:{\colon}                %% colon in  f: A -> B
\def\<#1>{\langle#1\rangle}   %% angle brackets

\def\then{\Rightarrow}
\def\D{{\cal D}}
\def\SDS{{\eightrm TDS}}

\outer\def\section#1. #2\par{%% Section divisions
      \bigskip\bigskip       %% space before new section
      \message{#1. #2}%      %% (for log file)
      \leftline{\bf#1. #2}%  %% boldface, left-justified
      \nobreak\smallskip     %% space after title
      \noindent}             %% next paragraph not indented


\outer\def\varsection#1\par{%%% for unnumbered sections
      \bigskip\bigskip       %% space before new section
      \message{#1 }%         %% (for log file)
      \leftline{\bf#1 }%     %% boldface, left-justified
      \nobreak\smallskip     %% space after title
      \noindent}             %% next paragraph not indented

\def\declare#1. #2\par{%    %% for defns, remarks, examples
      \medskip\noindent     %% space before new section
      {\bf#1.}\rm           %% bold header, roman text
      \enspace\ignorespaces %% space between header and text
      #2\par\smallskip}     %% space after paragraph

\def\cite#1{{\rm[#1]}}        %% reference citation
\def\eq#1{{\rm(#1)}}          %% print equation number
\def\opname#1{\mathop{\rm#1}\nolimits} %% operator name
\def\refno#1. #2\par{\smallskip\item{[#1]} #2\par}

%% Reference keys:

\def\Bastiani{1}
\def\Boman{2}
\def\Choquet{3}
\def\DonatoGeometrie{4}
\def\DonatoVirasoro{5}
\def\DonatoFibrations{6}
\def\Fro{7}
\def\Frolicherb{8}
\def\BFroli{9}
\def\Hamilton{10}
\def\Jarchow{11}
\def\Ke{12}
\def\Keller{13}
\def\Ckeller{14}
\def\Kri{15}
\def\Krieglb{16}
\def\Lang{17}
\def\Lawvere{18}
\def\Marinescu{19}
\def\Milnor{20}
\def\Seip{21}
\def\SouriauAlgoritme{22}
\def\Sou{23}
\def\Torre{24}
\def\TorreTangen{25}
\def\TorreBan{26}
\def\Wong{27}
\def\Yamamuro{28}

\newtoks\rightheadtext      %% running head for title
\newtoks\leftheadtext       %% running head for authors

\headline={\ifnum\pageno>1  %% no heading on first page
            \ifodd\pageno   %% title on odd pages
             \hfil \eightrm \the\rightheadtext \hfil
             \llap{\tenrm\folio}%
            \else \rlap{\tenrm\folio}%% authors on even pages
             \hfil \eightrm \the\leftheadtext \hfil \fi
           \else\hfil \fi}
\footline={\hfil}           %% pagenumbers on top only


\rightheadtext{Differentiability, Convenient Spaces}


\leftheadtext{CARLOS A. TORRE}



then $c$ is a $Lip^k$-curve iff $c$ is $j$-times
differentiable and $c^j$ is a $Lip^{k-j}$ curve if $0\leq j\leq k$.

The differential of a function $f\colon U\subset X \to Y$, where 
$(Y, Y^{\prime})$ is also preconvenient is defined as follows: $f$ is
called differentiable at $x$ in direction $v\in X$ if $c(t)= f(x+tv)$
is differentiable. This derivative is denoted $df(x,v)$ and $f$ is
called {\it differentiable} if $df(x,v)$ exists $\forall x\in U$, (if
$df$ is a $Lip^0$-map also, then $f$ is called {\it Lip-differentiable})
$\forall v\in X$. The {\it differential} of $f$ is the map
$df\colon U\times X \to Y$. And $f$ is called {\it $k$-times differentiable}
if $f$ is differentiable and $df(\cdot ,v)$ is $(k-1)$-times 
differentiable $\forall v\in X$, (if $f$ is Lip-differentiable and
$df$ is $(k-1)$-times Lip-differentiable $\forall v\in X$ then $f$ is
called {\it $k$-times Lip-differentiable}). In particular if $X, Y$ are
convenient spaces then these two definitions and the definition of
a $Lip^k$ map are equivalent. It is also equivalent to a stronger
condition of differentiability in which the limit exists uniformly
with respect to $x$ and $v$ and $f^{\prime}(x)\in L(E,F)$ where
$f^{\prime}(x)(v)= df(x,v)$ \cite\Seip (with respect to b-compact
sets: $K$ is b-compact in $E$ if there exists $B$ absolutly convex
such that $K$ is compact in
$E_B = \cup_{n\in \N}nB$).


\section 8. Convenient spaces and tangent diffeologies.

Given a pre-convenient space $(X, X^{\prime})$, a linear
tangent diffeology is defined on $X$ as follows: 
let $(X, P(X))$ be the diffeology
defined by $({\cal C}, {\cal F})$ and
let $ \sim$ be the canonical tangent diffeology defined by
$X^{\prime}$.

$(X, P(X), \sim)$ is linear: given $[c_1], [c_2]$ in $T_F^nX$, 
we define
$[c_1]+[c_2] = [c]$
where $c(t) = c_1(t) + c_2(t), c_i \in [c_i], i=1,2$,
this is well defined since
$D(f\circ c)\vert_0 = D(f\circ c_1)\vert_0 + D(f\circ c_2)\vert_0$,
$\forall f\in X^{\prime}$.

Let $\alpha \colon X \to T_FX$ be defined by
$\alpha (v_0) = [F+tv_0]_t $. Then $\alpha$ is linear by definition of
the linear structure on $T_FX$.

\declare Remark 8.1.

\item{[1]}
$\alpha$ is 1-1 (or $X\subset T_FX$) if and only if $(X, X^{\prime})$
is separated.
{\it Proof:}
If $(X, X^{\prime})$ is not Hausdorff  then $ X^{\prime}$ does not
separete points $\leftrightarrow \exists x_1, x_2\in X$
different such that $l(x_1) = l(x_2), \forall l\in X^{\prime}$ then
$ l\circ c_1 = l\circ c_2$, $\forall l\in X^{\prime}$,
where $c_i(t)= F + tx_i$, $i=1,2$, therefore
$Dl\circ c_1\vert_0 = Dl\circ c_2\vert_0 $ and then $[c_1] = [c_2]$. This
proves that $\alpha$ is not 1-1.
Assume now that $\alpha$ is not 1-1, then:
$\alpha (x_1) = \alpha(x_2)$ for some $x_1, x_2 \in X$. That is
$[F+tx_1] = [F+tx_2]$, then
$D(l\circ c_1) = D(l\circ c_2)$ for all $l\in X^{\prime}$, therefore
${d\over dt}l(F+tx_1)\vert_0 = {d\over dt}l(F+tx_2)\vert_0$, 
$\forall l\in X^{\prime}$,
then $l(x_1) = l(x_2)$ forall $l\in X^{\prime}$,
then $X^{\prime}$ does not separate points.
\qed

\item{[2]}
$\alpha$ is 1-1 and onto (or $X = T_FX$) if and only if $(X, X^{\prime})$
is a convenient space.
{\it Proof:}
Assume $(X, X^{\prime})$ is complete, then $\forall c\in {\cal C}$ the
weak derivative $c^{\prime}(t)$ exists, then
$D(l\circ c)(t_0) 
= l(c^{\prime}(t_0))
= Dl(F+tc^{\prime}(t))\vert_{t_0}, \forall l\in X^{\prime}$
then $[c] = [F+tc^{\prime}(t_0)] 
= \alpha (c^{\prime}(t)$
and therefore $\alpha$ is onto. Assume now that $\alpha$ is onto. Let
$c\in {\cal C}$ and let $[c] = \alpha(v_0)= [F+tv_0]$ where $v_0\in X$. 
Then
$D(l\circ c) = l(v_0)$, $\forall l\in X^{\prime}$.
Then $c^{\prime}(t)$ exists.
\qed

\item{[3]}
$(X, P(X), \sim)$ is continuous if $(X, X^{\prime})$ is convenient.
{\it Proof}:
Let $P_i(r,s), i=1,2$ be two 2-plaques such
that $p_1(r,0)= p_2(r,0)$. Identify $T_FX$ with $X$ and define
$$p(r,t) = p_1(r,0)+t([p_1(r,s)]_s + [p_2(r,s)]_s)$$
then $p(r,0)= p_1(r,0)$ and
$[p(r,t)]_t = [p_1(r,s)]_s + [p_2(r,s)]_s$.
Using the definitions it is proved that $p(r,t)$ is a 2-plaque.

\item{[4]}
If $(X, X^{\prime}), (Y, Y^{\prime})$ are convenient then
$D(X, Y) = {\cal M}(X, Y) = C^k_l(X, Y)$: we have that
$D(X,Y) = {\cal M}(X, Y)$ because $P{\cal M} = P{\cal M}^k_L$ and
$C^k_l(X, Y)\subset D(X,Y)$ from definition. If $f\in D(X, \R)$, then
$f\in Lip^k(X)$, therefore ${d\over dt}f(x+tv)\vert_0$ exists.

\item{[5]}
Conversely, a $P{\cal M}^k_L$ 
tangent diffeology $(X, P(X), \sim)$ is a convenient
space iff it is linear and $\forall F\in X$ the space $T_FX$ is
bijective with $X$, defining a sum on $X$ which is independent of $F$,
and with this operation $P(X)$ is generated by a subspace $X^{\prime}$
of linear functions $l\colon X \to \R$.

\section 9. Manifolds.

Let $\underline{{\cal V}^k}$ be a subcategory of the category of locally
convex vector spaces such that for any two objects $V, W$ the set
of morphisms $D^k(V,W)$ is a subspace of k-times weakly differentiable
maps $f\colon U\subset V \to W$, $U$ open. In particular
some examples are:
\item{a.}
Objets are Banach spaces and $D^k(V,W)$ is formed by $C^k$ Frechet
differentiable maps $f\colon U\subset V \to W$, $U$ open.
\item{b.}
Objects are locally convex vector spaces and $D^k(V,W)$ is the set of Gateaux
$C^k$ maps $f\colon U\subset V\to W$, $U$ open 
(k-times Gateaux differentiable and 
$f^k(x,v_1, \cdots v_k)$ is continuous as a map $U\times V^k \to W$)
\item{c.}
Objets are (pre)convenient spaces and $D^k(V,W) = Lip^k(V,W)$.
\item{d.}
Objects are the spaces $\R^n$, for each $n\in \N$ and
$D^k(\R^n ,\R^m)= P_n^m{\cal M}^k$, denoted $P{\cal V}^k$

A $\underline{{\cal V}^k}$-manifold modelled on a vector space $V$
is a set $M$ together with a set of bijective maps (called {\it charts})
$\phi_i\colon M_i\subset M \to V_i\subset V$, $i\in I$ such that
\item{1.}
$V_i$ is open for each $i\in I$ and $\cup_{i\in I}M_i=M$.
\item{2.}
$\phi_i(M_i\cap M_j)$ is open and $\phi_i\circ \phi_j^{-1}\in D^k(V,V)$
for all $i,j\in I$.
\item{3.}
The set of maps $\phi_i$ is maximal with respect to conditions 1,2.
A set of charts ${\cal A}$ satisfying 1,2 is called an {\it atlas}.

A map $f\colon X_1\to X_2$ between two $\underline{{\cal V}^k}$-manifolds
modelled on $V, W$ respectively
is called a $C^k$-map if $\phi_j\circ f\circ \phi_i^{-1} \in D^k(V,W)$ 
for every pair of charts $\phi_i, \phi_j$ in $X_1, X_2$ respectively.
The set of such $C^k$-maps is denoted $C^k(X_1, X_2)$.
Given a $\underline{{\cal V}^k}$-manifold $M$ modelled on $V$
with atlas ${\cal A}$,
a {\it tangent vector} at $x_0 \in M$ may be defined in one of the
following ways:
\item{[a]}
It is an equivalence class of pairs $(\phi_i, v)$ where $\phi_i\in {\cal A}$,
$v\in V$ and $(\phi_1, v_1) \sim (\phi_2, v_2)$ iff
$d(\phi_2^{-1}\circ \phi_1)\vert_0(v_1)=v_2$.
\item{[b]}
It is an equivalence class of $C^k$-curves $c\colon I\to M$ with $c(0)=x_0$:
choose any chart $\phi \in {\cal A}$ with $\phi(0)=x_0$, fixed, and
if $c_1, c_2$ are two curves, define $c_1\sim c_2$ iff
$$d(\phi^{-1}\circ c_1)\vert_0 = d(\phi^{-1}\circ c_2)\vert_0$$
\item{[c]}
It is an equivalence class of curves $c\colon I\to M$ with $c(x)= x_0$:
$c_1\sim c_2$ iff $d(f\circ c_1)\vert_0 = d(f\circ c_2)\vert_0$
for all $f\in D^k(M, \R)$
\item{[d]}
It is a derivation on the set of germs of functions in $D^k(M, \R)$ at 
$x_0$.

\declare Remark 9.1.

\item{[1]}
A topology is defined on a manifold $M$: $U\subset M$ is open iff
$\phi_i(U\cap M_i)$ is open $\forall i\in I$. Usually the topology is 
required to be Hausdorff and normal, and perhaps also paracompact in
order to have partitions of unity.

\item{[2]}
Definitions 1, 2, 3 of a tangent vector are equivalent and the set of
tangent vectors at $x_0$, denoted $T_{x_0}M$, is bijective with $V$. The
bijection is given by $\tau\colon V \to T_{x_0}M$, where 
$\tau(v)$ is $[\phi, v]$
for a fixed $\phi$ in definition 1, $[t\to \phi (\phi^{-1}(x_0+tv)]$
in definitions 2 and 3. Under definition 4, the space $T_{x_0}M$ contains
$V$: $\tau (v)f := df(\phi^{-1}(x_0)+tv)\vert_0$, and it is equal to $V$
in the category of Banach manifolds. 

\item{[3]}
If $M$ is a compact finite dimensional manifold, 
then the manifold structure may be recovered using only 
the algebra
$A= C^k(M)$: the set $M$ and its topology comes from Gelfand-Naimark
theorem ($M$ is the set of classes of irreducible representations of
$C^k(M)$ and its topology is the pointwise limit topology); having $M$,
we define the diffeology 
$P(M)$ as the set of plaques $p\colon U\subset \R^n \to M$, where
$U$ is open and $n\in \N$ such that $f\circ p\in  P{\cal V}^k$ for each
$f\in A$. The canonical tangent structure defined by $A$ allows the 
definition of $C^k$-maps. With this, the atlas ${\cal A}$ 
is the set of plaques
$p\colon U\to M_p$ such that $M_p\subset M$ is open, $p$ is a
homeomorphism and $p^{-1}$ is smooth.
The same construction works if $M$ is any manifold and we know not only
$A$ but also the set $M$. 

\item{[4]}
A similar problem is: given a set $M$ and an algebra 
$A$ of functions on $M$,
is $M$ a ${\cal V}^k$ manifold with algebra $A$?. A solution is:
the topology on $M$ and the set ${\cal M}$ is constructed 
as before, then the
answer is positive iff the collection of sets $M_p$ covers $M$. We may notice
that if $M$ is a manifold then the tangent structure is linear and continuous,
but it is not a sufficient condition (consider the sphere $S^2$ with the
diffeology $P(S^2)$ generated by ${\cal M}^k$ plaques along parallels, then the
algebra $A$ of ${\cal M}^k$ functions generates $P(S^2)$. The tangent
structure is linear and continuous. It is one dimensional everywhere,
except at poles where it is 2 dimensional. The topology is not compact 
and it is not a manifold.) It may be noticed also that 
if the tangent structure is linear and
continuous then the set $\Gamma (M)$ of smooth vector fields of $M$ is a
$A$ module (even if $M$ is not a manifold) 
and it must be a projective module if $M$ is a compact smooth manifold.


\item{[5]}
Every ${\cal V}^k$ manifold $M$ modelled on a vector space $V$ defines
a linear, continuous $\SDS$ in which
$P_1(M)$ is the set of $C^k$-maps $p\colon U\subset \R^n \to M$,
with the canonical tangent structure defined by $C^k(M, \R)$.
In general 
$$C^k(M) = {\cal C}^k_l(M) \subset {\cal C}^k(M)$$
and they are equal if $V$ satisfies that
$$\Phi \{ D^k(\R^n, V), n\in \N \} = D^k(M)$$
In this case $\underline{{\cal V}^k}$ is a subcategory of
$\underline{P{\cal M}}$ (for any two manifolds $M_1, M_2$ we have
$C^k(M_1, M_2) = {\cal C}^k(M_1, M_2)$). This occurs if $V$ is a $\SDS$,
in particular if $V$ is a convenient space, such as a Fr'chet space.
From remark 2 it follows that at each point both tangent spaces are
the same and isomorphic to $V$. Another $\SDS$ is defined by taking
$$P_2(M) = \{ p\colon u\subset \R^n \to M / f\circ p \in D^k(\R^n, \R), 
\forall f\in D^k(M) \}$$
We have $P_1(M) \subset P_2(M)$ and they are equal if
$$\Gamma (D^k(V, \R) = \{ D^k(\R^n, V), \forall n\in \N \}$$
In particular this holds if $V$ is a convenient space.


\varsection  Acknowledgments

\medskip
I gratefully acknowledge the support of the Vicerrector\'{\i}a de
Investigaci\'on of the University of Costa Rica. I would like also to
thank Joseph C. V\'arilly for helpful discussions.

\bigskip


\varsection  References

\frenchspacing

\refno \Bastiani.
Diff'rentiabilit' dans les espaces localement convexes. Districtures,
These Doct. Sci. Math. Fac. Sci. Univ. Paris 1962.


\refno \Boman.
J. Boman,
Differentiability of a function and of its compositions with
functions of one variable,
Math. Scand. 20, (1967) 249--68.

\refno \Choquet.
Choquet-Bruhat, De Witt-Morette, Dillard-Bleick,
Analysis, Manifolds and Physics,
Amsterdam, North Holland, 1982.

\refno \DonatoGeometrie.
P. Donato,
G\'eom\'etrie des orbites coadjointes des groupes de
dif\-feo\-mor\-phismes,
in: C. Albert, ed., {\it G\'eom\'etrie Symplectique et M\'ecanique},
Lecture Notes in Mathematics {\bf 1416} (Springer, Berlin, 1988)
84--104.

\refno \DonatoVirasoro.
P. Donato,
Les diffeomorphismes du circle comme orbit symplectique dans les
moments de Virasoro,
Preprint CPT--92/P.2681, CNRS--Luminy, 1992.

\refno \DonatoFibrations.
P. Donato and P. Iglesias,
Cohomologie des formes dans les espaces diffeologiques,
Preprint CPT--87/P.1986, CNRS--Luminy, 1987.

\refno \Fro.
A. Frolicher and A. Kriegl,
{\it Linear Spaces and Differentiation Theory\/},
(John Wiley, 1987).

\refno \Frolicherb.
A. Frolicher,
Durch Monoide erzeugte kartesisch abgeschlossene Kategorien,
Seminarberichte Fachbereich Math., Fernuniversitat Hagen, (1979) 7--48.

\refno \BFroli.
A. Frolicher and W. Bucher,
Calculus in Vector Spaces Without Norm,
Lect. Notes in Math. 30, Springer, Berlin, 1966. $N^{\circ}$ 4723.

\refno \Jarchow.
H. Jarchow,
Locally convex spaces,
Teubner, Stuttgart, 1981.

\refno \Ke.
H. Keller,
Differential calculus in locally convex spaces,
Lect. Notes Math. 417, 1974.

\refno \Keller.
H. Keller,
Raume stetiger multilinearer Abbildunger als Limesraume,
Math. Ann. 159, (1965) 259-270.

\refno \Ckeller.
H. Keller,
Ueber Probleme, die bei einer Differentialrechnung in
topologischen Vektorraumen auftreten, 
Festaband z. 70. Geburtstag v. Rolf Nevanlinna,
Springer Berlin (1966) 49-57.

\refno \Kri.
A. Kriegl,
Dierichtigen Raume fur Analysis im Unendlich-Dim.,
Monatshefte Math 94, (1982) 109--124.

\refno \Krieglb.
A. Kriegl,
A convenient setting of differential calculus in locally convex spaces,
Abh. Akad. Wiss. DDR, 2N, (1984) 135--40.

\refno \Lang.
S. Lang,
Introduction to Differentiable Manifolds,
Interscience Publ., Wiley, New York, 1962.


\refno \Lawvere.
Lawvere, L. W., Schanuel, S. H., Zame, W. R.,
On $C^{\infty}$-function spaces, Preprint (1981).

\refno \Marinescu.
G. Marinescu,
Espaces vectoriels pseudotopologiques et th'ories des distributions.
VEB Deutsch. Berlag d. Wissensch., Berlin, 1963.

\refno \Milnor.
J. Milnor, 
Remarks on infinite dimensional Lie groups in Relativity,
groups and Topology, Les Houches (1983),
1007-1057; North Holland, Amsterdam-New York (1984).

\refno \Seip.
U. Seip,
A convenient setting for differential calculus.
J. of Pure and Appl. Algebra 14 (1979) 73-100.

\refno \SouriauAlgoritme.
J. M. Souriau,
Un algoritme g\'en\'erateur de structures quantiques,
Ast\'erisque, hors s\'erie (1985) 341--399.

\refno \Sou.
J. M. Souriau,
Groupes diff'rentiels,
Lecture notes in math., 838 (1980) 91-128.

\refno \TorreTangen.
C. Torre,
A Tangent bundle on diffeological spaces,
Math/9801046 (1998).

\refno \Torre.
C. Torre,
Examples of smooth diffeological spaces,
Preprint (1999).

\refno \TorreBan.
C. Torre and A. Banyaga,
A symplectic structure on coadjoint orbits of diffeomorphism subgroups,
Ciencia y Tecnolog¡a 17 No 2, (1993) 1--14.

\refno \Wong.
Y. Wong,
Differential Calculus and Differentiable Partitions of Unity in
Locally Convex Spaces,
Univ. of Toronto, 1974.

\refno \Yamamuro.
S. Yamamuro,
Differential Calculus in Topological Linear Spaces,
Lect. Notes in Math. 374, Springer, Berlin, 1974.






\bye



